Simulation-Based Inference for Global Health Decisions

The COVID-19 pandemic has highlighted the importance of in-silico epidemiological modelling in predicting the dynamics of infectious diseases to inform health policy and decision makers about suitable prevention and containment strategies. Work in this setting involves solving challenging inference and control problems in individual-based models of ever increasing complexity. Here we discuss recent breakthroughs in machine learning, specifically in simulation-based inference, and explore its potential as a novel venue for model calibration to support the design and evaluation of public health interventions. To further stimulate research, we are developing software interfaces that turn two cornerstone COVID-19 and malaria epidemiology models COVID-sim, (https://github.com/mrc-ide/covid-sim/) and OpenMalaria (https://github.com/SwissTPH/openmalaria) into probabilistic programs, enabling efficient interpretable Bayesian inference within those simulators.

==> Makefile <==
NAME=main
PDFNAME=covid19-probprog-icml2020

all: clean build

build:
	pdflatex -jobname $(PDFNAME) $(NAME).tex
	make bib
	pdflatex -jobname $(PDFNAME) $(NAME).tex
	pdflatex -jobname $(PDFNAME) $(NAME).tex

bib:
	if [ -e $(PDFNAME).aux ] ; \
	then \
		echo COMPILE BIBTEX; \
		bibtex $(PDFNAME).aux; \
	else \
		echo NO REFERENCES TO COMPILE; \
	fi;

clean:
	rm -f $(PDFNAME).aux $(PDFNAME).bbl $(PDFNAME).log $(PDFNAME).out \
		$(PDFNAME).toc $(PDFNAME).blg $(PDFNAME).dvi $(PDFNAME).ps  \
		$(PDFNAME).nav $(PDFNAME).snm $(PDFNAME).vrb

